Evidence of Demographic rather than Ideological Segregation in News Discussion on Reddit

We evaluate homophily and heterophily among ideological and demographic groups in a typical opinion formation context: online discussions of current news. We analyze user interactions across five years in the r/news community on Reddit, one of the most visited websites in the United States. Then, we estimate demographic and ideological attributes of these users. Thanks to a comparison with a carefully-crafted network null model, we establish which pairs of attributes foster interactions and which ones inhibit them. Individuals prefer to engage with the opposite ideological side, which contradicts the echo chamber narrative. Instead, demographic groups are homophilic, as individuals tend to interact within their own group - even in an online setting where such attributes are not directly observable. In particular, we observe age and income segregation consistently across years: users tend to avoid interactions when belonging to different groups. These results persist after controlling for the degree of interest by each demographic group in different news topics. Our findings align with the theory that affective polarization - the difficulty in socializing across political boundaries-is more connected with an increasingly divided society, rather than ideological echo chambers on social media. We publicly release our anonymized data set and all the code to reproduce our results: https://github.com/corradomonti/demographic-homophily

==> alt-text.tex <==
Figure 1: \Description[Distribution of topics]{Distribution of topics across the selected submissions of r/news.}

Figure 2: \Description[Matrix of coefficients for interactions between demographic features on r/news in 2016]{Matrix of logistic regression coefficients for interactions between all pairs of demographic features obtained for the r/news subreddit in 2016 by the socio-demographic features model. We show only coefficients that are significant in at least 4 years out of 5.}

Figure 3: \Description[Coefficients for homophiliac and heterophilic interactions over time for the SD model]{Plot of logistic regression coefficients for homophiliac and heterophilic interactions over time between socio-demographic features obtained (independently) for each year in the r/news subreddit in the SD model.}

Figure 4: \Description[Coefficients for homophiliac and heterophilic interactions over time for the SD+T model]{Plot of logistic regression coefficients for homophiliac and heterophilic interactions over time between socio-demographic features obtained (independently) for each year in the r/news subreddit in the SD+T model.}

Figure 5: \Description[Coefficients for interactions between demographic features and topics]{Logistic regression coefficients for interactions between demographic features and topics obtained for the r/news subreddit in 2016 by the SD+T model. Filled disks indicate associations significant in at least 4 years out of 5.}

